Primordial black hole formation and abundance: contribution from the non-linear relation between the density and curvature perturbation

The formation and abundance of primordial black holes (PBHs) arising from the curvature perturbation $\zeta$ is studied. The non-linear relation between $\zeta$ and the density contrast $\delta$ means that, even when $\zeta$ has an exactly Gaussian distribution, significant non-Gaussianities affecting PBH formation must be considered. Numerical simulations are used to investigate the critical value and the mass of PBHs which form, and peaks theory is used to calculate the mass fraction of the universe collapsing to form PBHs at the time of formation. A formalism to calculate the total present day PBH abundance and mass function is also derived. It is found that the abundance of PBHs is very sensitive to the non-linear effects, and that the power spectrum $\mathcal{P}_\zeta$ must be a factor of $\sim2$ larger to produce the same number of PBHs as the linear model (where the exact value depends on the critical value for a region to collapse and form a PBH). This also means that the derived constraints on the small-scale power spectrum from constraints on the abundance of PBHs are weaker by the same factor.

==> Sections/Section5.tex <==

\section{Masses of primordial black holes}

\todo{Produce a plot of the mass of the resultant black hole against to the amplitude of the perturbation that produced it. Again, we'll want to use several different profile shapes, and I'm not sure how we will want to parameterise the perturbation amplitude - so a data file containing all final masses and input parameters will be useful.}

\todo{Relation of comoving wavenumber $k$ to a horizon mass/radius.}

